Incorporating Domain Knowledge into Medical NLI using Knowledge Graphs

Recently, biomedical version of embeddings obtained from language models such as BioELMo have shown state-of-the-art results for the textual inference task in the medical domain. In this paper, we explore how to incorporate structured domain knowledge, available in the form of a knowledge graph (UMLS), for the Medical NLI task. Specifically, we experiment with fusing embeddings obtained from knowledge graph with the state-of-the-art approaches for NLI task (ESIM model). We also experiment with fusing the domain-specific sentiment information for the task. Experiments conducted on MedNLI dataset clearly show that this strategy improves the baseline BioELMo architecture for the Medical NLI task.

==> Conclusion.tex <==
\section{Conclusion}
In this paper, we showed that knowledge graph embeddings obtained through applying state-of-the-art model like DistMult from UMLS could be a promising way towards incorporating domain knowledge leading to improved state-of-the-art performance for the medical NLI task. We further showed that sentiments of medical concepts can contribute to medical NLI task as well, opening a new direction to be explored further. With the emergence of knowledge graphs in different domains, the proposed approach can be tried out in other domains as well for future exploration.

==> ExperimentalResults.tex <==
\begin{flushleft}
\begin{table}[!thb]
\centering
\begin{tabular}{ll}
\hline
Model        & Accuracy \\ \hline
fastText & 68.7\% \\
GloVe & 73.1\% \\
$BioELMo$~\cite{jin2019probing} & 78.2\% \\
$ESIM w/ K$~\cite{lu2019incorporating} & 77.8\% \\ 
\hline
fastText w/ KG+Sentiment & 73.67\% \\
GloVe w/ KG+Sentiment & 74.46\% \\
BioELMo w/ KG & 78.76\% \\
\textbf{BioELMo w/ KG+Sentiment}         & \textbf{79.04\%}   \\ \hline
\end{tabular}
  \vspace{-0.2cm}
\caption{Performance of our models (bottom four) along with the state-of-the-art baseline models (top four). Baseline results for fastText, GloVe are obtained from ~\citet{romanov-shivade-2018-lessons}. Adding knowledge graph information to the base models showed an absolute improvement of 4.97\% in case of fastText and 1.36\% in case of GloVe. The baseline model utilizing BioELMo as base embeddings~\cite{jin2019probing} showed an accuracy of 78.2\%. On adding knowledge graph information, we were able to improve these results to 78.76\% and on further addition of sentiment information, the accuracy rose to 79.04\%}
\label{table:2}
\end{table}
  \vspace{-0.5cm}
\end{flushleft}

\section{Experimental Results and Analysis}

As discussed earlier, we mainly consider the models presented by~\citet{jin2019probing} [$BioELMo$] and~\citet{lu2019incorporating} [\textbf{$ESIM w/ K$}] as our baselines. We report accuracy as the performance metric. Table~\ref{table:2} represents the performance comparison of our proposed models and the baselines, which shows that incorporation of knowledge graph embeddings helps to improve the model performance. All the results reported use ESIM as their base model. Further, incorporating sentiment of medical concepts gives further improvements, achieving an overall ~1\% improvement over the baseline model. 

We also see from ~\cite{jin2019probing} that BERT and BioBERT show an accuracy of 77.8\% and 81.7\%, respectively. However, they also showcase through a probing task that BioELMo is a better feature extractor than BioBERT, even though the latter has higher performance when fine tuned on MedNLI. Due to this reason, we take BioELMo as our base architecture and use our enhancements over BioELMo instead of BioBERT.

We also experimented with using fastText and GloVe as our base general embeddings. With addition of Knowledge Graph embeddings and sentiment information, the results showed an absolute improvement from 68.7\% to 73.67\% in case of fastText, and 73.1\% to 74.46\% in case of GloVe. All results are summarized in Table~\ref{table:2}.

\noindent\textbf{Training Details: }
For \textit{DistMult}, we use word embeddings dimensions to be 100. SGD was used for optimization with an initial learning rate of $10^{-4}$. The batch size was set to 100. For \textit{ESIM}, we take the dimension of hidden states of BiLSTMs to be 500. We set the dropout to 0.5 and choose an initial learning rate of $10^{-3}$. We choose a batch size of 32 and run for a maximum of 64 epochs. The training is stopped when the development loss does not decrease after 5 subsequent epochs.

\if{1}
\begin{table*}[t]
\centering
\begin{tabular}{>{\footnotesize}l>{\footnotesize}l>{\footnotesize}l>{\footnotesize}l>{\footnotesize}l}
\hline
Premise & Hypothesis & gold label & BioELMo & BioELMo w/ Knowledge & BioELMo w/ Knowledge+Sentiment\\ \hline
History of CVA. & patient has history of stroke & entailment & neutral & entailment \\
Blood glucose 626. & Patient has normal A1c & contradiction & entailment & contradiction \\
\multicolumn{1}{m{2cm}} She does admit to some diarrhea at home. & The patient is constipated & contradiction & entailment & contradiction & contradiction \\ \hline
Per report ECG with initial qtc of 410 now 475., QRS 82 initially, now 86 rate= 95. & Patient has angina & neutral & neutral & entailment \\
PAST MEDICAL HISTORY:  Type 2 diabetes mellitus. & the patient has type 1 diabetes & contradiction & entailment & entailment & entailment \\ \hline
\end{tabular}
\caption{Error Analysis}
\label{table:3}
\end{table*}

\if{0}
p: No recent change in bowel or bladder habits.
h: The patient does not have a urinary tract infection.

Example for sentiment information mattering. Here, gold label=neutral, bioelmo=entailment, bioelmo+KG=entailment, bioelmo+KG+sentiment=neutral.

Negated concepts:
p: None
h: ``Urinary Tract Infection

\fi
\subsection{Results}
Our hypothesis is that adding extra structured domain knowledge will improve the accuracy and therefore, we mainly compare BioELMo with BioELMo w/ KG (proposed model). BioELMo w/ KG achieves an accuracy of 78.76\%. All the results shown in this paper are calculated on the test dataset.

By including sentiment information obtained from MetaMap to the BioELMo w/ KG model, we achieved 79.04\% accuracy. 
\fi

\if{0}
p: The patient ruled out for a myocardial infarction; however, he was transferred to [**Hospital1 58**] for cardiac catheterization.
h: The patient did not have an acute STEMI

Example for sentiment information mattering. Here, gold label=entailment, bioelmo=entailment, bioelmo+KG=contradiction, bioelmo+KG+sentiment=entailment.

Negated concepts: 
p: ``myocardial infraction'' (heart attack)
h: ``Acute STEMI'' (very serious type of heart attack)

Only issue is that bioelmo marked it as entailment, no clue why. But can we say that since this was a direct link in KG, we can say that it was classified correctly with confidence?
\fi

\noindent\textbf{Qualitative Analysis: }We explain the efficacy of our model with the help of a few examples. Consider the sentence pair, $p$: ``History of CVA'' and $h$: ``patient has history of stroke''. In medical terms, `CVA' means `Cerebrovascular accident' which is another term for `stroke'. By Using MetaMap, we are able to find that the preferred term for `stroke' is `Cerebrovascular accident' and hence our model classified the sample pair correctly as entailment. %To take another example, consider the pair $p$: ``The patient ruled out for a myocardial infarction; however, he was transferred to [**Hospital1 58**] for cardiac catheterization.'' and $h$: ``The patient did not have an acute STEMI''. The 

% Positive #2
In many cases, our baseline models fail to capture negative sentiment present in the premise or hypothesis. For example, in case of $p$: Watermelon stomach with gastric varices, without bleed in more than 2 years, $h$: Patient has no active bleeding, BioELMo predicts this as contradiction, whereas the gold label is entailment. But, by using the negative sentiment, captured by Metamap, for the word `bleed' in both premise and hypothesis, our model is able predict the label correctly. 
% \footnote{For visualization of the cross-attentions between $p$ and $h$ in our models, we have also provided the attention maps from ESIM, for few of the examples above, in the Appendix.} 
%which further solidifies the analysis above.)

% Positive #3
% In the case of $p$: The patient remained hemodynamically stable and was admitted for further workup. $h$: the patient is hypotensive, we observe that the baseline model wrongly predicts the label, as it is not able to connect the words `hemodynamically' and `hypotensive' in the ESIM attention map, which we suspect to be because of lack of a good representation of the keywords. (We draw this conclusion 

%The level of blood glucose indicated is higher than normal. `A1c' is a common blood test used to diagnose type 1 and type 2 diabetes. Since the patient has higher blood glucose level, the patient having normal `A1c' would be a contradiction and is thus classified as such. 
%\todo{Better explanation or remove datapoint}
%\section{Error Analysis}
On the other hand, even though our model produces promising improvement over state-of-the-art performance, there are cases for which our model is not able to classify correctly. For the sentence pair $p$: ``She was speaking normally at that time'' and $h$: ``The patient has no known normal time where she was speaking normally.'' contradicting each other, our model predicts this to be entailment. The probable reason could be that, the negative sentiment associated with ``speaking normally'' is not captured by MetaMap and the noise in MetaMap is percolated further. %The negative sentiment associated with ``speaking normally'' is also not captured by MetaMap. 
In another example case, $p$: ``He had no EKG changes and first set of enzymes were negative.'' and $h$: ``the patient has negative enzymes.'' our model classifies this pair as entailment while the gold label is neutral. While the premise says that the first set of enzymes was negative, it gives no information about the current state. This leads us to believe that a sense of timeline is extremely important for examples like this which is not already being captured by our model. Taking care of these cases would be our immediate future work.

%Premise: "He was mentally alert and was ambulating without difficulty at the facility." Hypothesis: "the patient was unable to ambulate" Here MetaMap fails to assign a negative sentiment with ambulate and therefore, while the gold label is contradiction, all the models predicted this to be an entailment. Since the term ambulate appears in both premise and hypothesis, the BioELMo and BioELMo w/ KG create an association between them. However, this should have been correctly classified by BioELMo w/ KG + Sentiment, however due to misclassification of sentiment associated with ambulate in hypothesis by MetaMap, the model failed to perform.

%We have listed a few more datapoints and the outputs for the two models in table 2.

%*put sample erroneous cases for different set-ups along with proper insights*

==> Introduction.tex <==
\section{Introduction}
Natural language inference (NLI) is one of the basic natural language understanding tasks which deals with detecting inferential relationship such as entailment or contradiction, between a given premise and a hypothesis. In recent years, with the availability of large annotated datasets like SNLI~\cite{bowman-etal-2015-large}, MultiNLI~\cite{williams2018broad}, researchers have come up with several neural network based models which could be trained with these large annotated datasets and are able to produce state-of-the-art performances~\cite{bowman-etal-2015-large,bowman2016fast, munkhdalai2017neural,sha2016reading,chen2017enhanced,tay2017compare}. With these attempts, even though NLI in domains like fiction, travel etc. has progressed a lot,
NLI in medical domain is yet to be explored extensively. With the introduction of MedNLI~\cite{romanov-shivade-2018-lessons}, an expert annotated dataset for NLI in the clinical domain, researchers have started pursuing the problem of clinical NLI. Modeling informal inference is one of the basic tasks towards achieving natural language understanding, and is considered very challenging. 
MedNLI is a dataset that assists in assessing how good a sentence or word embedding method is for downstream uses in medical domain.

Recently, with the emergence of advanced contextual word embedding methods like ELMo~\cite{peters2018deep} and BERT~\cite{devlin2018bert}, performances of many NLP tasks have improved, setting state-of-the-art performances. 
Following this stream of literature, ~\citet{lee2019biobert} introduce BioBERT, which is a BERT model pre-trained on English Wikipedia, BooksCorpus and fine-tuned on PubMed (7.8B tokens in total) corpus, PMC full-text articles. ~\citet{jin2019probing} propose BioELMo which is a domain-specific version of ELMo trained on 10M PubMed abstracts, and attempt to solve medical NLI problem with these domain specific embeddings, leading to state-of-the-art performance. These two attempts show a direction towards solving medical NLI problem where the pretrained embeddings are fine-tuned on medical corpus and are used in the state-of-the-art NLI architecture.

~\citet{chen2018neural} proposed the use of external knowledge to help enrich neural-network based NLI models by applying Knowledge-enriched co-attention, Local inference collection with External Knowledge, and Knowledge-enchanced inference composition components. Another line of solution tries to bring in the extra domain knowledge from sources like Unified Medical Language System (UMLS)~\cite{bodenreider2004unified}. ~\citet{romanov-shivade-2018-lessons} used the knowledge-directed attention based methods in ~\cite{chen2018neural} for Medical NLI. Another such attempt is made by~\citet{lu2019incorporating}, where they incorporate domain knowledge in terms of the definitions of medical concepts from UMLS with the state-of-the-art NLI model ESIM~\cite{chen2017enhanced} and vanilla word embeddings of Glove~\cite{pennington2014glove} and fastText~\cite{bojanowski2017enriching}. Even though, the authors achieve significant improvement by incorporating only concept definitions from UMLS, the features of this clinical knowledge graph are yet to be fully utilized. Motivated by the emerging trend of embedding knowledge graphs to encode useful information in a high dimensional vector space, we propose the idea of applying state-of-the-art knowledge graph embedding algorithm on UMLS and use these embeddings as a representative of additional domain knowledge with the state-of-the-art medical NLI models like BioELMo, to investigate the performance improvement on this task. Additionally, we also incorporate the sentiment information for medical concepts given by MetaMap ~\cite{metamap} leading to further improvement of the performance.  
Note that, as state-of-the-art baselines, we use the models proposed by~\citet{jin2019probing} and~\citet{lu2019incorporating}. Since, both of these studies consider ESIM as the core NLI model which makes it more convenient for us to incorporate extra domain knowledge and to have a fair performance comparison with these state-of-the-art models.        
Our contributions are two-fold.
\begin{itemize}%[noitemsep,nolistsep,leftmargin=*]
    \item We incorporate domain knowledge via knowledge graph embeddings applied on UMLS. We propose an intelligent path-way to combine contextual word embeddings with the domain specific embeddings learnt from the knowledge graph, and feed them to the state-of-the-art NLI models like ESIM. This helps to improve the performance of the base architecture.
    \item We further show the usefulness of the associated sentiments per medical concept from UMLS in boosting the performance further, which in a way shows that if we can carefully use the domain knowledge present in sources like UMLS, it can lead to promising results as far as the medical NLI task is concerned. 
\end{itemize}


==> Methodology.tex <==
\section{Dataset}
In this study, we use the MedNLI dataset ~\cite{romanov-shivade-2018-lessons}, a well-accepted dataset for natural language inference in clinical domain. The dataset is sampled from doctors' notes in the clinical dataset MIMIC-III~\cite{mimic-iii} and is arguably the largest publicly available database of patient records. The entire dataset consists of 14,049 premise-hypothesis pairs divided into 11,232 train pairs, 1,395 validation pairs and 1,422 test pairs. Each such pair consists of a gold label which could be either entailment (true), contradiction (false), or neutral (undetermined). The average (maximum) sentence lengths of premises and hypotheses are 20 (202) and 5.8 (20), respectively.

\section{Proposed Approach}
The task is to classify the given premise ($p$) and hypothesis ($h$) sentence pair into one of the three classes: entailment, contradiction and neutral. Following the approach by~\citet{jin2019probing}, we use the BioELMo embedding model where authors bring in contextual information in terms of embeddings obtained via applying ELMo trained on 10M PubMed abstracts, and use these with the state-of-the-art ESIM model~\cite{chen2017enhanced} for the NLI task. The architecture includes two sentence encoders each of which takes in as input the word embeddings of $p$ and $h$. The inputs are run through corresponding bi-directional LSTM encoder layers. Pairwise attention matrix is computed between encoded $p$ and $h$, which forms the attention layer followed by a second bi-directional LSTM layer run separately over $p$ and $h$. Max and average pooling are performed over the outputs of LSTM layers and the output of pooling operations is run through a softmax model. 
We feed this architecture an additional domain knowledge from UMLS as vector representations obtained via knowledge graph embeddings, the details of which are described below. \\   

\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{emnlp-ijcnlp-2019-latex/model.jpg}
  \vspace{-0.2cm}
  \caption{\textbf{BioELMo w/ KG pipeline} Here $w$ is the NLTK tokenized form of premise (p) or hypothesis (h), $ph$ is the MetaMap tokenized form of sentence (p or h). $s$ signifies the sentiment vector. $e^w$ and $e^d$ signify the aligned word embeddings and DistMult embeddings, respectively. $s'$ signifies the aligned sentiment vector.}
  \label{fig:model}
  \vspace{-0.5cm}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{emnlp-ijcnlp-2019-latex/esim.jpg}
    \vspace{-0.2cm}
    \caption{Aligned premise and hypothesis embeddings are obtained using the method described in Figure \ref{fig:model} and become inputs to the ESIM model.}
    \label{fig:esim}
  \vspace{-0.5cm}
\end{figure}

\noindent\textbf{UMLS: } Unified Medical Language System (UMLS) is a compendium which includes many health and biomedical vocabularies and standards. It provides a mapping structure between these vocabularies and is a comprehensive thesaurus and ontology of biomedical concepts. UMLS contains 3 knowledge sources: Metathesaurus, Semantic Network, and Specialist Lexicon and Lexical Tools. We use two of these sources: the Metathesaurus and the Semantic Network. The Metathesaurus comprises of over 1 million biomedical concepts and 5 million concept names. 
Each concept has numerous relationships with each other. 
Each concept in the Metathesaurus is assigned one or more Semantic Type linked to other Semantic Types through a semantic relationship. This information is provided in the Semantic Network of UMLS. There are 127 semantic types and 54 relationships in total. Semantic types include ``disease", ``symptom", ``laboratory test" and semantic relationships include ``is-a", ``part-of", ``affects". \\

\noindent\textbf{MetaMap: } MetaMap is a tool for effective entity mapping of biomedical text to the concepts and semantic type in UMLS Metathesaurus. On feeding a sentence to MetaMap, it divides the sentence into phrases based on medical concepts found in the sentence and for each medical concept it provides its unique ID in Metathesaurus, its position in the sentence, the list of semantic types the concept is mapped to, the preferred medical name and unique ID for the preferred concept (such as a concept called ``chest pain'' would be mapped to its preferred medical term ``angina''). We also get a boolean value associated with each concept denoting whether the medical concept occurs in a negative sentiment (1) or not (0). For example, in the sentence, ``The patient showed no signs of pain", the medical concept `pain' would appear with a negative sentiment. Note that, for each extracted phrase, there may be more than one related medical concepts and each concept may have more than one possible mapping. For our study, we only consider the mapping with the highest MetaMap Indexing (MMI) score, a metric provided by MetaMap. As a result, every word in a sentence has zero or one corresponding medical concept.

\textbf{Constructing the appropriate knowledge graph:} We use the MetaMap tool to process the complete MedNLI dataset and extract the relevant information from UMLS into a smaller knowledge graph.  

First, we use MetaMap to extract medical concepts from $p$ and $h$, and map them to the standard terminology in UMLS. We choose to map each medical concept to its preferred medical term. E.g., ``blood clots'' would map to ``thrombus''. This helps us to map different synonymous surface forms to the same concept. This results in 7,496 unique medical concepts from UMLS matched to various words and phrases in the MedNLI dataset. Each unique concept in UMLS becomes a node in our knowledge graph. The relations in our knowledge graph come from two sources: The Metathesaurus and the Semantic Network of UMLS. 

Using relations extracted from these two sources, we connect the filtered medical concepts from UMLS to build a smaller Knowledge Graph (subgraph of UMLS). 

We get 117,467 triples from the Metathesaurus and 23,824,105 triples from the Semantic Network, which constitute the edgelists in the prepared knowledge graph.

\textbf{Knolwedge Graph Embeddings:} To obtain the embedding from this graph, we use state-of-the-art DistMult model~\cite{distmult2015}. The choice is inspired by ~\citet{kadlec-etal-2017-knowledge}, which reports that an appropriately tuned DistMult model can produce similar or better performance while compared with the competing knowledge graph embedding models. DistMult model embeds entities (nodes) and relations (edges) as vectors. It uses a matrix dot product to measure compatibility between head ($h$) and tail ($t$) entities, connected by a relation ($r$). Logistic loss is used for training the model.

\begin{equation}
    \sigma_{DistMult}(h, r, t) = r^T(h \cdot t)
\end{equation}

\if{0}
\begin{table}[t]
\centering
\begin{tabular}{ll}
\hline
Model        & Accuracy \\ \hline
ELMo    & 75.8\%         \\
BioELMo & 78.2\% \\ 
FastText & 77.8\% \\ \hline
\end{tabular}
\caption{Baseline Results as obtained from ~\cite{jin2019probing} and ~\cite{lu2019incorporating}}
\label{table:1}
\end{table}
\fi

\textbf{Combining Knolwedge Graph Embeddings with BioELMo:}
As explained in Figure \ref{fig:model}, each sentence ($p$ or $h$) is tokenized using the simple module of NLTK\footnote{\url{https://www.nltk.org/}} as well as processed using MetaMap to get UMLS concepts. To align these, we copy the UMLS concept for a phrase to all the constituent words.\\
Once we have aligned the tokens obtained via NLTK and MetaMap, we apply BioELMo and DistMult to get the embedding vectors, \(e_{BioELMo,w}\) and \(e_{DistMult,w}\) for each word $w$. We concatenate these vectors as \(e_{w} = e_{BioELMo,w} \oplus e_{DistMult,w}\), to obtain the word representation for $w$. We call the proposed model which uses these embeddings as \textit{BioELMo w/ KG}.

\textbf{Combining Sentiment Information:} We further enhance the domain knowledge by incorporating sentiment information for a concept separately. For that purpose, we use the sentiment boolean provided by MetaMap and create a 1-d vector $(sent_w)$ containing 0 for positive medical concepts or non-medical concept and 1 for negative concept. This 1-d vector is aligned with the \(e_{DistMult,w}\) in the same fashion as explained above. We concatenate this single dimension with our concatenated resultant embeddings. Thus \(e_{w} = e_{BioELMo,w} \oplus e_{DistMult,w} \oplus sent_w\). We call the proposed model which uses these embeddings as \textit{BioELMo w/ KG + Sentiment}.

We use the vanilla ESIM model ~\cite{chen2017enhanced} and feed the obtained concatenated embeddings for each word in the premise and hypothesis to the model, to be trained for the inference task (see Figure~\ref{fig:esim}).
